Exact schedulability test for sporadic mixed-criticality real-time systems using antichains and oracles

This work addresses the problem of exact schedulability assessment in uniprocessor mixed-criticality real-time systems with sporadic task sets. We model the problem by means of a finite automaton that has to be explored in order to check for schedulability. To mitigate the state explosion problem, we provide a generic algorithm which is parameterised by several techniques called oracles and simulation relations. These techniques leverage results from the scheduling literature as "plug-ins" that make the algorithm more efficient in practice. Our approach achieves up to a 99.998% reduction in the search space required for exact schedulability testing, making it practical for a range of task sets, up to 8 tasks or maximum periods of 350. This method enables to challenge the pessimism of an existing schedulability test and to derive a new dynamic-priority scheduler, demonstrating its good performance. This is the full version of an RTNS 2024 paper.

==> content/102_tasket_table.tex <==
% \begin{table}[ht]
%       \centering
%       \caption{Task set $\tau^{a}$.}
%       \scalebox{1.0}{% Adjust scale factor as needed
%       \begin{tabular}{c|cc}
%                    & $\tau_1$ & $\tau_2$ \\ \hline
%         $C_i(\lo)$ & $1$      & $1$      \\
%         $C_i(\hi)$ & $2$      & $1$      \\
%         $T_i$      & $2$      & $2$      \\
%         $D_i$      & $2$      & $2$      \\
%         $L_i$      & $\hi$    & $\lo$
%       \end{tabular}
%       }
%       \label{table:taskset-example}
% \end{table}

\begin{table}[t]
      \centering
      \caption{Task set $\tau^{a}$.}
    \vspace{-10pt}
      % \scalebox{1.0}{% Adjust scale factor as needed
      \begin{tabular}{l|ccccc}
      \hline
         & $C_i(\lo)$ & $C_i(\hi)$ & $T_i$ & $D_i$ & $L_i$ \\ \hline
$\tau_1$ & $1$        & $2$        & $2$   & $2$   & $\hi$ \\
$\tau_2$ & $1$        & $1$        & $2$   & $2$   & $\lo$ 
      \end{tabular}
      % }
      \label{table:taskset-example}
\end{table}

==> content/501_idle_task_simulation_proof.tex <==
\begin{proof}
  Let $S_1, S^\scom_1$ and $S_2$ be three states in $\States{\tau}$ s.t. $(S_1,
  S^\scom_1) \in E$ and $S_1 \idle S_2$, let us show that there exists $S^\scom_2 \in
  \States{\tau}$ with $(S_2, S^\scom_2) \in E$ and $S^\scom_1 \idle S^\scom_2$.

  Let $S^\sreq_1$ and $S^\srun_1 \in \States{\tau}$
  and $\tau^\sreq \subseteq \tau $ be such that : $S_1 \RqTrans{\tau^\sreq} S^\sreq_1
  \CtTrans{\schedule(S^\sreq_1)} S_1^\srun \CpTrans{\schedule(S^\sreq_1)} S_1^\scom$. Those exist by
  \autoref{auto} and since $(S_1, S_1^\scom) \in E$.

  First, observe that, by \autoref{def:idle}, $\Eligible{S_1}\subseteq\Eligible{S_2}$. 
  So, by \autoref{treq}, there exists a $\tau^\sreq$-release transition 
  from $S_2$. Let $S_2^\sreq$ be the state s.t. $S_2 \RqTrans{\tau^\sreq} S_2^\sreq$. 
  By \autoref{treq}, again, it is easy to check that $S_1^\sreq\idle S_2^\sreq$.  
  
    Next, let us show that we can simulate the run transition from $S_2^\sreq$. To alleviate notations, 
    let us denote, from now on, 
    $\schedule(S^\sreq_1)$ by $\run_1$ and $\schedule(S^\sreq_2)$ by $\run_2$. Let us consider 
    $\run_1=\schedule(S^\sreq_1)$, which can be either $\run_1\in\Active{S^\sreq_1}$ or $\bot$. 
    If $\run_1\in\Active{S^\sreq_1}$, we already know that $\run_1\in\Active{S^\sreq_2}$ too. 
    Moreover, since the scheduler is deterministic, we have $\run_1=\run_2$,
    by \autoref{run}. So in both cases, we can let $S_2^\srun$ be the state s.t. $S^\sreq_2
    \CtTrans{\run_2} S_2^\srun$. Finally, by \autoref{def:idle} and~\ref{run}, 
    it is easy to check that $S_1^\srun\idle S_2^\srun$.

 Finally, let us show that we can simulate the signal transitions from $S_1^\srun$. Let us observe $S_1^\scom$. By \autoref{tcom}, there are four possibilities, keeping in mind that  $\run_1=\run_2$
 \begin{enumerate}
    \item When $\run_1=\bot$ or $\run_1\in\Completed{S^\srun_1}$, in which case 
    $S^\scom_1=S^\srun_1$.
    In the first case, we have $\run_2=\bot$. In the latter case, we have 
    $\run_2\in\Completed{S^\srun_2}$ since $S^\srun_1\idle S^\srun_2$. In both cases, we conclude
    that the signal transition will have the same effect on $S^\srun_2$ than on $S^\srun_1$, i.e. 
    $S^\srun_2\CpTrans{\run_2}S^\scom_2$ with $S^\scom_2=S^\srun_2$, 
    hence $S^\scom_1\idle S^\scom_2$, trivially.
    \item Else when $\run_1$ signals completion in $S^\srun_1$. Hence, the same task can signal completion from
    $S^\srun_2$ since $S^\srun_1\idle S^\srun_2$. 
    Thus, $S^\srun_1\CpTrans{\run_1}\sigCmp{S^\srun_1}{\run_1}$ and 
    $S^\srun_2\CpTrans{\run_2}\sigCmp{S^\srun_2}{\run_2}$. 
    It is easy to check that $\sigCmp{S^\srun_1}{\run_1}\idle\sigCmp{S^\srun_2}{\run_2}$.
    \item Else if $\rct_{S^\srun_1}(\run_1)=0$, we have 
    $\rct_{S^\srun_2}(\run_2)=0$ as well since $S^\srun_1\idle S^\srun_2$. 
    In this case, we have $S^\srun_1\CpTrans{\run_1}\critUp{S^\srun_1}{\run_1}$ 
    and $S^\srun_2\CpTrans{\run_2}\critUp{S^\srun_2}{\run_2}$, 
    and it is easy to check that 
    $\critUp{S^\srun_1}{\run_1}\idle\critUp{S^\srun_2}{\run_2}$.
    \item Otherwise, in the last case, we have $S^\srun_1\CpTrans{\run_1}S^\scom_1$
    with $S^\srun_1=S^\scom_1$. Since $S^\srun_1\idle S^\srun_2$, we have
    $S^\srun_2\CpTrans{\run_2}S^\scom_2$ 
    with $S^\srun_2=S^\scom_2$ as well. Hence $S^\scom_1\idle S^\scom_2$.
 \end{enumerate}

  To conclude the proof, it remains to prove that $S_1 \idle S_2$ and $S_1 \in
  \DeadlineMiss{\tau}$ implies that $S_2 \in \DeadlineMiss{\tau}$ too.
  %
  Let $\tau_i$ be such that $\rct_{S_1}(\tau_i) > 0 \wedge \ttd_{S_1}(\tau_i) \leq 0$.
  %
  Since $S_1 \idle S_2$ : $\rct_{S_2}(\tau_i) = \rct_{S_1}(\tau_i)$ and $\nat_{S_2}(\tau_i)
  \leq \nat_{S_1}(\tau_i)$, thus $\ttd_{S_2}(\tau_i) \leq \ttd_{S_1}(\tau_i)$.
  %
  Hence $\rct_{S_2}(\tau_i) > 0 \wedge \ttd_{S_2}(\tau_i) \leq \ttd_{S_1}(\tau_i)
  \leq 0$ and therefore $S_2 \in \DeadlineMiss{\tau}$ as per~\autoref{fail}.
\end{proof}

==> header/authors_ieee.tex <==
\author{
\IEEEauthorblockN{Simon Picard}
\IEEEauthorblockA{\textit{Ourway} \\
Brussels, Belgium \\
snspicard@gmail.com}
\and
\IEEEauthorblockN{Antonio Paolillo}
\IEEEauthorblockA{\textit{Vrije Universiteit Brussel} \\
Brussels, Belgium \\
antonio.paolillo@vub.be}
\and
\IEEEauthorblockN{Gilles Geeraerts}
\IEEEauthorblockA{\textit{Université libre de Bruxelles} \\
Brussels, Belgium \\
gilles.geeraerts@ulb.be}
\and
\IEEEauthorblockN{Joël Goossens}
\IEEEauthorblockA{\textit{Université libre de Bruxelles} \\
Brussels, Belgium \\
joel.goossens@ulb.be}
}
